Reading Rational Univariate Representations on lexicographic Groebner bases

In this contribution, we consider a zero-dimensional polynomial system in $n$ variables defined over a field $\mathbb{K}$. In the context of computing a Rational Univariate Representation (RUR) of its solutions, we address the problem of certifying a separating linear form and, once certified, calculating the RUR that comes from it, without any condition on the ideal else than being zero-dimensional. Our key result is that the RUR can be read (closed formula) from lexicographic Groebner bases of bivariate elimination ideals, even in the case where the original ideal that is not in shape position, so that one can use the same core as the well known FGLM method to propose a simple algorithm. Our first experiments, either with a very short code (300 lines) written in Maple or with a Julia code using straightforward implementations performing only classical Gaussian reductions in addition to Groebner bases for the degree reverse lexicographic ordering, show that this new method is already competitive with sophisticated state of the art implementations which do not certify the parameterizations.

==> 0_abstract.tex <==
 In this contribution, we consider a zero-dimensional polynomial system in $n$ variables defined over an effective field $\mathbb{K}$.
 We propose a practical Las Vegas algorithm for computing a Rational Univariate Representation (RUR) of its solutions without any condition on the ideal other than being zero-dimensional. Our key result is that the RUR can be read (using a closed formula) from lexicographic Gr\"{o}bner bases of bivariate elimination ideals, even when the original ideal is not in shape position, so that a simple algorithm similar to the well-known FGLM method can be used. In particular, we address the problem of certifying whether a linear form is a separating form for the given system, also using a closed formula from the Gr\"obner bases. In our experiments, we show that this certification procedure can be used to produce sparse separating forms with small coefficients, and observe that this generally leads to parametrizations that can be computed more efficiently.
 
%  {\color{red} Old version:}
%  In the context of computing a Rational Univariate Representation (RUR) of its solutions, we address the problem of certifying a separating linear form and, once certified, calculating the associated RUR, without any condition on the ideal other than being zero-dimensional. Our key result is that the RUR can be read (using a closed form formula) from lexicographic Gr\"{o}bner bases of bivariate elimination ideals, even in the case where the original ideal that is not in shape position, so that one can use the same core as the well known FGLM method to propose a simple algorithm. Our first experiments, either with a very short code (300 lines) written in Maple or with a Julia code using  straightforward implementations performing only classical Gaussian reductions in addition to Groebner bases for the degree reverse lexicographic ordering, show that this new method is already competitive with sophisticated state of the art implementations which do not certify the parameterizations.
 
